Gaussian-Bernoulli RBMs Without Tears

We revisit the challenging problem of training Gaussian-Bernoulli restricted Boltzmann machines (GRBMs), introducing two innovations. We propose a novel Gibbs-Langevin sampling algorithm that outperforms existing methods like Gibbs sampling. We propose a modified contrastive divergence (CD) algorithm so that one can generate images with GRBMs starting from noise. This enables direct comparison of GRBMs with deep generative models, improving evaluation protocols in the RBM literature. Moreover, we show that modified CD and gradient clipping are enough to robustly train GRBMs with large learning rates, thus removing the necessity of various tricks in the literature. Experiments on Gaussian Mixtures, MNIST, FashionMNIST, and CelebA show GRBMs can generate good samples, despite their single-hidden-layer architecture. Our code is released at: \url{https://github.com/lrjconan/GRBM}.

==> sections/fig_sampling.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}{.99\textwidth}
    \centering
    \begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
    \includegraphics[width=.124\linewidth]{imgs/MNIST_sampling/img_000001.png} 
    &
    \includegraphics[width=.124\linewidth]{imgs/MNIST_sampling/img_000005.png} 
    &
    \includegraphics[width=.124\linewidth]{imgs/MNIST_sampling/img_000010.png} 
    &
    \includegraphics[width=.124\linewidth]{imgs/MNIST_sampling/img_000020.png} 
    &
    \includegraphics[width=.124\linewidth]{imgs/MNIST_sampling/img_000030.png} 
    &    
    \includegraphics[width=.124\linewidth]{imgs/MNIST_sampling/img_000040.png} 
    &        
    \includegraphics[width=.124\linewidth]{imgs/MNIST_sampling/img_000050.png} 
    &
    \includegraphics[width=.124\linewidth]{imgs/MNIST_sampling/img_000100.png}
    \\
    \multicolumn{1}{c}{(a)} & \multicolumn{1}{c}{(b)} & \multicolumn{1}{c}{(c)} & \multicolumn{1}{c}{(d)} & \multicolumn{1}{c}{(e)} & \multicolumn{1}{c}{(f)} & & 
    \end{tabular}
\end{subfigure}
\caption{Sampling process of Gibbs-Langevin.}
\label{fig:sampling}
\end{figure}
